Transfer Learning for Information Extraction with Limited Data

This paper presents a practical approach to fine-grained information extraction. Through plenty of experiences of authors in practically applying information extraction to business process automation, there can be found a couple of fundamental technical challenges: (i) the availability of labeled data is usually limited and (ii) highly detailed classification is required. The main idea of our proposal is to leverage the concept of transfer learning, which is to reuse the pre-trained model of deep neural networks, with a combination of common statistical classifiers to determine the class of each extracted term. To do that, we first exploit BERT to deal with the limitation of training data in real scenarios, then stack BERT with Convolutional Neural Networks to learn hidden representation for classification. To validate our approach, we applied our model to an actual case of document processing, which is a process of competitive bids for government projects in Japan. We used 100 documents for training and testing and confirmed that the model enables to extract fine-grained named entities with a detailed level of information preciseness specialized in the targeted business process, such as a department name of application receivers.

==> text/1_1_Related_Work.tex <==
\section{Related Work}\label{sec:related_work}

Conventional methods utilize dictionaries \cite{watanabe2007graph} or take advantage of machine learning for named entity extraction. Recently, the success of deep learning attracts researchers to apply this technique to information extraction. A recent study employs Long-Short Term Memory (LSTM) with a Conditional Random Field (CRF) to classify the contextual expressions \cite{lample2016neural}. Several research projects focus on the nested named entities and have a great progress so far~\cite{finkel2009nested,ju2018neural}. 

%The non-dictionary approaches can dramatically reduce the efforts of maintaining data, yet it still requires training data annotation efforts because of the nature of supervised learning.

For NER, high-level concepts such as people, places, organizations usually need to extract. However, for practical applications, categories must be in a more detailed level \cite{JJAndrew2018legal}. Here, fine-grained entity type classification was proposed, especially in the field of question answering, information retrieval \cite{lee2006fine,shimaoka2016attentive}, or the automatic generation of ontology \cite{fleischman2002fine}. However, the main challenge of fine-grained NER is the amount of training data required to train the classifier. To tackle this problem, transfer learning \cite{transferlearning} is an appropriate solution. It leverages pre-trained models trained by a large amount of out-domain data to build a new model with a small number of training data in a new domain. Transfer learning is efficient because we daily have faced with limited training data. Let's take our scenario as an example, we need to extract values for 24 tags in long Japanese documents while the number of the training documents is only 78. Thus, transfer learning is one of the most efficient technique in such scenario \cite{shin2016deep,weiss2016survey}. 
% There are three types of transfer as follows:
% \begin{itemize}
%     \item Neural networks as fixed feature extractor: The last fully connected layer is removed and the rest is used as a fixed feature extractor for the new dataset. After obtaining the feature vectors, we can apply various algorithms to learn.
%     \item Fine-tuning the network: The final layer is replaced in compatible with the new dataset. The classifier is fine-tuned the weights by continuing the training procedure. In some scenarios, we can fix some earlier layers and only fine-tune higher-level portion of the network.
%     \item Pretrained models: Since training networks takes a long time and consumes multiple resources. It is common to save some checkpoints and continue training the network from the checkpoints.
% \end{itemize}

One of the highlights of transfer learning is the recent open source named Bidirectional Encoder Representation from Transformers (BERT) \cite{devlin2018bert}. BERT is a form of transfer learning and has achieved state-of-the-art results on 11 NLP tasks, including the very competitive Stanford Question Answering Dataset (SQuAD). In this work, we develop a model based on BERT for our business task, which extracts information in long Japanese documents. 


==> text/1_introduction.tex <==
\section{Introduction}\label{sec:intro}

The recent growth of AI technologies is dramatic, as many applications have already been deployed to real business cases \cite{mckinsey}. One of the most significant topics in the business scene is the conversion of unstructured text into structured one because it is stated as an entrance to the digital transformation \cite{william2007unstructured,digitaltransformation}. It has been studied by many proposed methods \cite{nlp}. In business services, the extraction of specific information matters such as organization names, personal names, addresses, or date plays an important role to facilitate document processing systems. Therefore, named entity recognition (NER) is one of the key technologies which help AI software contributes to the commercial applications \cite{ner2}.

NER has been received attention due to its important role \cite{lample2016neural,finkel2009nested,ju2018neural}. Conventional approaches use dictionary-based \cite{ner2}, which requires a huge amount of time to set up to keep it up-to-date. Recent approaches have been utilized machine learning to reduce the efforts of dictionary building and maintenance \cite{lample2016neural}. Majority of the researches successfully have done the simple tasks of NER, yet those have focused on relatively-easy tasks; hence it is not always straightforward to apply the proposed algorithms to real cases due to two gaps. The first gap is about the amount of data. Document processing typically focuses on narrow, specific topics rather than general, wide ones, where only a small amount of annotated data is available. It challenges neural-network-based natural architectures, which usually require more than 10,000 annotated training examples. For instance, CoNLL 2003 provided 20,000 annotated words for NER \cite{devlin2018bert}. For actual cases, in a narrow domain, annotating the such number of training data is a non-trivial task. For the second gap, the identification of information types cannot be merely the categories \cite{fleischman2002fine,lee2006fine,shimaoka2016attentive}. The usual scope of NERs is to extract the categories of information such as organization names; however, in many cases, there can be two types of organizations, such as payee and payer in invoices. We believe that this level of detailed understanding is the key to the practical use of NER.\vspace{-0.3cm}

\begin{figure}[!h]
    \centering
  \includegraphics[width=8cm]{figure/system.png}
  \caption{The overview of the system.}\vspace{-0.2cm}
  \label{fig:system}
\end{figure}

%without using a dictionary,
In this research, we aim to identify a particular type of named entities from documents with the limited amount of training data. The proposed model utilizes the idea of transfer learning to fine-grained NER tasks. As shown in Figure \ref{fig:system}, the information extractor employs BERT \cite{devlin2018bert} for addressing the small number of training data (the first gap) and then stacks CNN with multilayer perceptron (MLP) to extract detail information, e.g. the year of procurement and the name of institution (the second gap). Outputs are stored in the JSON format for other tasks of document processing in our system. Our contributions are two-fold:
\begin{itemize}
    \item We propose a practical model of fine-grained NER which employs BERT \cite{devlin2018bert} as an element of transfer learning \cite{transferlearning}. By employing BERT and retraining the model with a small amount of data, our model achieves significant improvements compared to strong methods in extracting fine-grained NER. To the best our knowledge, we are the first study for the extraction of fine-grained NER for Japanese bidding documents.
    \item We present the actual case of applications which have been demanded by one Japanese electricity supplier and confirmed that the accuracy of the proposed model is acceptably high enough for practical use. 
\end{itemize}

We applied our model to a real scenario of extracting information from bidding documents. Statistical analyses show that our model with small training data achieves improvements in term of F-score compared to strong baselines.
%Experimental results indicate that our model has ability to extract high-quality information with a small number of training data.

%The rest of the paper is organized as follows: Section \ref{sec:related_work} presents the relevant research. Our proposed model is described in Section \ref{sec:the_model}. Conducting experiments to verify the model is specified in Section \ref{sec:experiment}. We show the results, discussion, and error analysis in Sections \ref{sec:results} and \ref{sec:error-analysis}. Section \ref{sec:conclusion} concludes our investigations.



==> text/2_Approaches.tex <==
\begin{table}[!h]
  \caption{Information need to be extracted from bidding contract documents. Content type of name can be the name of an entity such as a company, department, or person.}
  \includegraphics[width=8.2cm]{figure/content.png}\vspace{-0.5cm}
\small
\label{table:tags}
\end{table}

\begin{figure*}[!h]
    \centering
  \includegraphics[width=17cm]{figure/BERT_CNN.pdf}\vspace{-0.1cm}
  \caption{The BERT-CNN model for extracting the value of a tag.} \vspace{-0.4cm}
  \label{fig:BERT_CNN}
\end{figure*}

\section{Proposed Approach} \label{sec:the_approach}
This section first introduces the problem and then describes our proposed model for information extraction from very long texts of Japanese bidding documents with limited training data.

\subsection{Task Definition}
This research focuses on an actual case of document processing which is competitive bids for government projects in Japan. The task is to extract values for fields (tags) from bidding documents of an electric power company. A bidding document is a long document which has 3 sections 1) specifications, 2) invitation to bid, 3) instructions to bid.  
\begin{figure}
  \includegraphics[width=8.2cm]{IEEECS_CPS_LaTeX_Letter_2Col/figure/bidding_doc.PNG}
    \caption{A part of bidding document. Clause 3 (two first lines) mean ''\textit{supply period from 04/01/2019 to 03/31/2020} (MM/dd/YYYY)".} \vspace{-0.5cm}
\label{fig:bidding_doc_example}
\end{figure}

Table \ref{table:tags} shows target information to be extracted. As observed, many tags may have the same value or data types, e.g. deadlines for the questionnaire (tag 14) and bidding (tag 16). Hence, locating the value of a specific tag is challenging and needs to understand the context in the document.

Figure \ref{fig:bidding_doc_example} shows a part of a bidding document with three clauses 3, 4, 5 of the specification section. The yellow highlighted texts are the values for tag 6 (start date of procurement), and tag 7 (end date of procurement).
%Another difficulty is that a tag is not represented by specific terms. Therefore, to retrieve the values correctly, the learning model need to understand the document structures and meaning of text.

% For example, given a paragraph like Figure~\ref{fig:example}
% \begin{figure}
%   \includegraphics[width=8.2cm]{figure/example.png}
%     \caption{Example of a document.}
% \label{fig:example}
% \end{figure}

% , the yellow line is the value of tags 20, 22, and the green line is the value of tags 18, 21, 23, 24.

\subsection{Proposed Model}\label{sec:model_architecture}
Figure \ref{fig:BERT_CNN} shows the overall architecture of the proposed model. The model has three main components: (i) the input vector representations of input tokens, (ii) BERT for learning hidden vectors for every token from the input tag and the document, and (iii) a convolution layer for capturing the local context and a softmax to predict the value location. The rest of this section will describe all parts of the model. 

\subsubsection{Input representation}\label{sec:input_representation}
Each input data includes the tag and the bidding document. The tag is treated as a single sequence, and the document is split into segments with the length of 384 tokens. Each token vector representation is determined based on the embeddings of token, sequence, and position. To differentiate among the input sequences, a special token (SEP) is inserted between them. For example, as showed in Figure \ref{fig:BERT_CNN}, the tag $i$ has $N_i$ tokens, in which $token_1$ corresponds to embedding $E^i_1$. The document has $k$ sequences separated by token [SEP]. Most of the specification of embeddings follows the original paper \cite{devlin2018bert}.

\subsubsection{BERT}
BERT is a multi-layered bidirectional Transformer encoder, which allows our model to represent the context of a word by considering its neighbors \cite{devlin2018bert}. This is unlike unidirectional models that learn the contextual representation for each word using the words in one side (left of right). For example, considering the word ``bank" in two sentences ``I went to the bank to deposit some money" and "I went to the bank of the river", the representations of ``bank" are identical for a left-context unidirectional model, but they are distinguished with the use of BERT. This characteristic is compatible with our problem where many tags have homogeneous values. Let's take a look to Table \ref{table:tags}, given an address, it may be the address for demand (tag 5), submitting the application of qualification (tag 20), submitting for of bid (tag 22), or place of the opening bid (tag 24). Therefore, in our problem, the context aspect is critical to determine the tag that the address belongs to.

In our research, a pre-trained BERT was employed for two reasons. Firstly, BERT has shown state-of-the-art performance on many NLP tasks ranging over single/pair sentence classification, question answering, and sentence tagging. We, therefore, take advantage of BERT for our task of information extraction. Secondly, a pre-trained model is a suitable solution to tackle our scenario of lacking training data. More precisely, we received only 100 documents for training and testing from our client. This is unpractical to train the whole network from scratch. To tackle this problem, we decided to use BERT as a type of transfer learning to fine-tune our model on bidding documents.

\subsubsection{Convolutional layer}\label{sec:cnn}
A convolutional layer was stacked on the top of BERT to learn local information of its input. Applying BERT is to take advantages of data in other domain, and produces hidden vectors from the tag and the bidding document. For this reason, the hidden vectors are for common texts that the network was pre-trained. To adapt to our domain, the convolutional layer is the essential component for capture statistical patterns. 

\subsubsection{Information extraction}\label{sec:information_extraction}
We formulate the information extraction problem as a question answering task. The value is pulled from the document by querying the tag. In the model, BERT learns the context of the document given the tag and produces hidden vectors for every token; the convolutional layer adjusts the vectors towards to our domain. Finally, a softmax layer is used to predict the location of the value. Each token is predicted to one of three outcomes including the start/end positions, and irrelevant to the tag. The extracted value is gathered based on the start to end positions with the highest probabilities.

\subsubsection{Training}\label{sec:training}
Training our model includes two stages: (i) pre-training and (ii) fine-tuning. For the first stage, the pre-trained weights of BERT were reused, while the weights of the rest layers were randomly initialized. The BERT was trained with a large text corpus of Japanese collected from Wikipedia. The training task is to predict whether a sentence is the next or just a random of other sentence \cite{devlin2018bert}.

The whole network was fine-tuned in 20 epochs with our training data by using cross-entropy. We used multilingual BERT-based model trained for 102 languages on a huge amount of texts from Wikipedia. The model has 12 layers, a hidden layer of 768 neurons, 12 heads and 110M parameters. Convolution uses 768 filters with the window size = 3.

==> text/3_Experiments.tex <==
\section{Settings and Evaluation Metric}\label{sec:experiment}

\subsection{Dataset}
The dataset contains 100 bidding documents of a Japanese electric power company, in which 78 documents were used for training and 22 documents for testing.
%Table \ref{table:datastatistics} shows the statistics of the dataset.

\begin{table}[ht!]
\centering
\caption{Statistics of the dataset.}
\begin{tabular}{lcc}
\hline
Statistics & mean & Std. \\ \hline
\#training samples & 78 & - \\
\#testing samples & 22 & - \\
\#characters/sample & 22,537 & 17,191 \\
\#sentences/sample & 616 & 368 \\ \hline
\end{tabular}
\label{table:datastatistics}
\end{table}

From Tables \ref{table:tags} and \ref{table:datastatistics}, we can observe that the extraction extracts many similar types of short values in a very long document, which has an average of 616 sentences.

\subsection{Baselines}
To verify the efficiency of our approach, we compare our model to five baselines as follows.
%, including: (i) the basic model of BERT; (ii) $n$-grams features with MLP;  (iii) a deep neural network which is trained from scratch using Glove as word embedding.
\begin{itemize}
    \item \textbf{BERT}: is the basic model which obtains state-of-the-art performance on many natural language processing tasks, including QA \cite{devlin2018bert}. We directly applied BERT for QA on our testing data, without any additional training.
    
    \item \textbf{BERT+CRF}: stacks CRF on BERT for prediction. This is because CRF is a conventional method for information extraction and NER. This method was trained on training data and then applied to test data.
    
    \item \textbf{BERT+LSTM+CRF}: This model uses LSTM to capture the hidden representation of sequences and employs CRF for classification. This is a variation of LSTM-CRF for NER \cite{lample2016neural}. We also tried with BiLSTM but its results are not good to report.
    
    \item \textbf{$n$-grams+MLP+regex}: was trained with $n$-gram features ($n$ in $[1, 4]$). The MLP was used to predict the paragraph containing the values of tags. The regular expression was finally applied to extract the values. 
    %This method requires a \textit{dictionary} of possible texts referring to the tags.
    
    \item \textbf{Glove+CNN+BiLSTM+CRF}: We used a deep neural network including layers of convolution, bidirectional Long Short Term Memory (BiLSTM), and conditional random fields (CRFs) to automatically extract tags of input texts. For token embedding, we use Glove \cite{pennington2014glove}.

\end{itemize}

\subsection{Evaluation metric}
We used F-score (F-1) to evaluate the performance of our model as well as the baselines. We matched extracted outputs to ground-truth data to compute precision, recall, and F-score. The final F-score was computed on all tags.

==> text/4_Result_and_Discussion.tex <==
\section{Results and Discussion}\label{sec:results}
Table \ref{table:f1_scores} reports the comparison according to F1-score. On average, our method outperforms others notably. Our model exploits the efficiency of BERT trained on a large amount of data; therefore, it can potentially capture the hidden representation of data. By stacking convolution and retraining the model with 78 training documents, our model has the ability to adapt to a new domain. As a result, the model can correctly extract information on bidding documents and can improve the performance over BERT-QA of 4.55\%. The improvements come from two possible reasons: (i) we employ BERT for limited training data and (ii) we take advantage of CNN for fine-tuning to capture local context. This confirms our assumption in Section \ref{sec:intro} that we can utilize transfer learning for information extraction in a narrow domain with limited data.

\begin{table}[ht!]
\centering
\caption{Comparison of methods according F1-score}
\begin{tabular}{lc}
\hline
Method & Avg. of F1 \\ \hline
BERT (QA)  & 0.8607 \\
BERT+CRF & 0.1773 \\
BERT+LSTM+CRF & 0.3817 \\
BERT+CNN+MLP (Our model)  &\textbf{ 0.9062} \\ \hline
$n$-grams+MLP+Regex & 0.8523 \\
CNN+BiLSTM+CRF+MLP & 0.6766\\ \hline
\end{tabular}\vspace{-0.2cm}
\label{table:f1_scores}
\end{table}

The BERT-QA model is the second best. It is understandable that this model also uses BERT as a pre-trained model to extract hidden representation. However, it needs to be adapted to a new domain. It shows the efficiency of retraining the model on a new domain. Even with a small amount of data (78 training documents), our model can improve the F-score. Interestingly, BERT-CNN and BERT-LSTM-CNN do not show improvements. The possible reason is bidding documents are very long (Table \ref{table:datastatistics}); therefore, long-term dependencies may affect these models. The model using MLP with $n$-grams features achieves competitive results. This is because this model uses two steps to extraction candidates. The first step uses MLP to detect whether a sentence contains extracted information or not. The second step uses regular expressions to extract candidates. However, in some cases, the expressions cannot cover the patterns of text (please refer to Section \ref{sec:error-analysis}). An interesting point is that the model CNN-BiLSTM+MLP outputs low scores, in which its performance is lower than $n$-grams+MLP of 17.57\%. As mentioned above, training deep neural networks from scratch with limited data is difficult to convergence because we need to optimize a large number of parameters. The feature-based method requires less training data but it easily suffers from the definition of regular expressions.

%There are two possible reasons. The first one is that this model uses Glove as word embedding; however, Glove is trained for general domain, not for bidding documents. The second reason is that this model is applied directly to the test data, without retraining. As a result, the difference between two domains makes a challenge for this model.

We observed F-score on each tag to analyze how each model works. To do that, we matched extracted text to reference and compute scores, which are plotted in Figure \ref{fig:f1_scores}. We did not plot the results of BERT-CRF, BERT-LSTM-CRF, and CNN due to its low scores.
\begin{figure}[ht!]
    \centering
  \includegraphics[width=8.2cm]{figure/F1_Scores.PNG}
  \caption{F1-scores per tag.}\vspace{-0.2cm}
  \label{fig:f1_scores}
\end{figure}
As can be seen, our model works stably on all tags, and usually achieves the best F1 scores in comparison with BERT-QA and $n$-grams-MLP. This again supports results in Table \ref{table:f1_scores} where our model is the best. It should be noted that the feature-based method obtains 0\% of F1 for tag 10 (classification of reserved electric energy). The reason is that $n$-grams features and the regular expressions may not capture well the patterns of reserved electric energy (tag 10). This shows that the $n$-grams+MLP+regex method can be affected by the definition of regular expressions. As the result, it could not find any values for tag 10 on the test set. By contrast, our model trained on BERT can exploit rich hidden representation from large pre-trained data and with 78 training documents of bids, the model can correctly extract tag 10.

%The efficiency of transfer learning is also confirmed from Table \ref{table:f1_scores} and Figure \ref{fig:f1_scores}.  

\section{Error Analysis}\label{sec:error-analysis}
In this section, we investigate how our model works on real data of bids. We observed the output of our model and the baselines. Table \ref{table:error analysis} shows some predicted values for three tags 21, 22, 23 (\ref{table:tags}) in documents of two contracts.
\begin{CJK}{UTF8}{min}
\begin{table*}[!h]
\setlength{\tabcolsep}{3pt}
\small
\caption{Some examples of model outputs. The correct answers and correct predictions are highlighted in blue. We did not show outputs of BERT, BERT-CRF and BERT-LSTM-CRF due to space limitation.}
\label{table:error analysis}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{lL{3.5cm}L{3.5cm}L{3.5cm}L{6cm}}
\hline
Tag & $n-gram$-MLP & Our model & CNN-BiLSTM & Correct answer \\ \hline
File & 九州0553 &  &  &  \\
21 & (232)6118 & {\color[HTML]{3531FF} 宮崎県会計管理局物品管理調達課物品調達担当} & 目1番地10郵便番号882－ & {\color[HTML]{3531FF} 宮崎県会計管理局物品管理調達課物品調達担当}  (Miyazaki Prefecture Accounting Administration Department Goods Management Procurement Section Goods Procurement) \\
22 & 目1番地10郵便番号882-0853電話番号098 & {\color[HTML]{3531FF} 〒882-0835延岡市新小路2丁目1番地10} & 延岡市新小路2丁 & {\color[HTML]{3531FF} 〒882-0835延岡市新小路2丁目1番地10} (postal code 882-0835 Miyazaki, Nobeoka, Shinkoji, 2 Chome−1−10) \\
23 & (232)6181 & {\color[HTML]{3531FF} 宮崎県会計管理局物品管理調達課物品調達担当} & 延岡市新小路2丁 & {\color[HTML]{3531FF} 県立延岡病院総務課整備担当} (Prefectural Nobeoka Hospital General Affairs Division Maintenance Section) \\ \hline
File & 中国0041 &  &  &  \\
21 & {\color[HTML]{3531FF} 岡山市東区役所瀬戸支所1階総務民生課} & 瀬戸支所総務民生課 & 岡山市東区瀬戸町瀬戸45番地岡山市東区役所瀬戸支所宛 & {\color[HTML]{3531FF} 岡山市東区役所瀬戸支所1階総務民生課} (Okayama City Higashi Ward Office Seto Branch 1F General Affairs and Welfare Division) \\
22 & {\color[HTML]{3531FF} 〒700－0899備前瀬戸郵便局留} & 岡山市東区瀬戸町瀬戸45番地 & 〒700-0899備前瀬戸郵便局留岡山市役所東区役所瀬戸支所宛 & {\color[HTML]{3531FF} 〒700－0899備前瀬戸郵便局留} (Bizen Seto Post Office Station, postal code: 700－0899) \\
23 & 岡山市役所東区役所瀬戸支所宛 & 瀬戸支所総務民生課 & 〒700-0899備前瀬戸郵便局留岡山市役所東区役所瀬戸支所宛 & {\color[HTML]{3531FF} 岡山市役所東区役所瀬戸支社} (Okayama City Hall Higashi Ward Office Seto Branch Office) \\ \hline
\end{tabular}\vspace{-0.5cm}
% }
\end{table*}
\end{CJK}
% \begin{figure*}[ht!]
% \captionof{table}[]{Some examples of model outputs. The correct answers and correct predictions are highlighted in blue.}
%     \centering
%   \includegraphics[width=16cm]{figure/error_analysis.pdf}
%   \label{table:error analysis}
% \end{figure*}

After observing, we found that for the feature-based method, it may suffer from the out of vocabulary problem because regular expressions were created by on keywords defined by humans. Although the classifier can predict correctly the sentence containing the value, the regular expression fails to locate the information. Taking the contract 0553 as an example, since the address of the company is not in the training data, the regular expression only captures the number part. Unlikely, the deep models can predict both the text and number parts in this case. However, the model trained from scratch usually produces uncompleted text, especially with the long-text values. This comes from the lack of training data that is one of the essential keys to allow the convergence of a deep model. In contrast, the pre-trained model can predict the whole content.

We also found that the feature-based methods can predict short values like date times, and numbers efficiently. In this case, the classifier finds the sentence using features and the regular expression can locate the information easily. For these types of fields, the performance of the feature-based and the deep models is similar. This is shown in Figure \ref{fig:f1_scores}.  
\section{Conclusion}
\label{sec:conclusion}
We presented a transfer learning method for information extraction with limited data. In the experiment, we used 100 documents for the training and validation, and confirmed that our method achieves high accuracy of fine-grained classification with the limited number of annotated data. We believe that the result implies a positive aspect of the concept of transfer learning for real information extraction scenarios.

A possible direction of our research is to investigate more final layers for classification. We also encourage to add heuristic features generated from humans and change the structure of our model by replacing CNN by more deeper structures, e.g. CNN-BiLSTM.
